Towards Modernising Data Collection and Archive for the Tor Network

CollecTor is developed by Tor Project's Metrics Team for the purpose of archiving data relating to the public Tor network and applications developed by Tor Project. This report distills the requirements for a prototype modernized replacement of the CollecTor service, and evaluates frameworks and libraries that are available to reduce code maintenance costs for the CollecTor service.

==> Makefile <==
all:
	dot -Tpdf reference-checker.dot > reference-checker.pdf
	dot -Tpdf architecture.dot > architecture.pdf
	pdflatex modern-collector.tex
	bibtex modern-collector
	pdflatex modern-collector.tex
	pdflatex modern-collector.tex
	-[ `hostname` = "z" ] && \
	  scp modern-collector.pdf people.torproject.org:public_html/volatile/

